Short Packets over Block-Memoryless Fading Channels: Pilot-Assisted or Noncoherent Transmission?

We present nonasymptotic upper and lower bounds on the maximum coding rate achievable when transmitting short packets over a Rician memoryless block-fading channel for a given requirement on the packet error probability. We focus on the practically relevant scenario in which there is no \emph{a priori} channel state information available at the transmitter and at the receiver. An upper bound built upon the min-max converse is compared to two lower bounds: the first one relies on a noncoherent transmission strategy in which the fading channel is not estimated explicitly at the receiver; the second one employs pilot-assisted transmission (PAT) followed by maximum-likelihood channel estimation and scaled mismatched nearest-neighbor decoding at the receiver. Our bounds are tight enough to unveil the optimum number of diversity branches that a packet should span so that the energy per bit required to achieve a target packet error probability is minimized, for a given constraint on the code rate and the packet size. Furthermore, the bounds reveal that noncoherent transmission is more energy efficient than PAT, even when the number of pilot symbols and their power is optimized. For example, for the case when a coded packet of $168$ symbols is transmitted using a channel code of rate $0.48$ bits/channel use, over a block-fading channel with block size equal to $8$ symbols, PAT requires an additional $1.2$ dB of energy per information bit to achieve a packet error probability of $10^{-3}$ compared to a suitably designed noncoherent transmission scheme. Finally, we devise a PAT scheme based on punctured tail-biting quasi-cyclic codes and ordered statistics decoding, whose performance are close ($1$ dB gap at $10^{-3}$ packet error probability) to the ones predicted by our PAT lower bound. This shows that the PAT lower bound provides useful guidelines on the design of actual PAT schemes.

==> Inputs/defs.tex <==
\usepackage{bm}
\usepackage{upgreek}
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{mathrsfs}
\usepackage{xspace}

\safemath{\mi}{I}
\safemath{\difent}{\mathrm{h}}		%differential entropy
\safemath{\NonnegReal}{\mathbb{R}^{+}}


\safemath{\indist}{\cdfP} %input distribution
\safemath{\outdist}{\cdfQ} %output distribution
\safemath{\inpdf}{\pdfp} %input pdf
\safemath{\outpdf}{\pdfq} %output pdf
\safemath{\testdist}{\cdfP} %the distribution of test P_{Z|W}

%\safemath{\tr}[#1]{\mathrm{tr}\left\lbrace #1  \right\rbrace}

\safemath{\powallocvec}{\vecv}
\safemath{\powalloc}{v}
\safemath{\encoder}{f} % the encoder of the code
\safemath{\decoder}{g} % the decoder of the code
\safemath{\msg}{J} % the message
\safemath{\csir}{\mathrm{r}}
\safemath{\csit}{\mathrm{t}}
\safemath{\csi}{\mathrm{csi}}
\safemath{\csirt}{\mathrm{rt}}
\safemath{\Rcsirt}{R_{\csirt}} %rate with CSIT
\safemath{\Rcsir}{R_{\csir}}
\safemath{\Rcsit}{R_{\csit}}
\safemath{\cohblock}{T}
\safemath{\blocklength}{n}
\safemath{\selbranches}{L}


\safemath{\Rnocsit}{R_{\mathrm{no}}} %rate without CSIT
\safemath{\Rnocsi}{R_{\mathrm{no}}} %rate without CSIT
\safemath{\Rgeneral}{R_{\mathrm{no,rt}}} %rate with general CSI condition
\safemath{\equalR}{R_{\mathrm{e}}}

\newcommand*\pFqskip{8mu}
\catcode`,\active
\newcommand*\pFq{\begingroup
        \catcode`\,\active
        \def ,{\mskip\pFqskip\relax}%
        \dopFq
}
\catcode`\,12
\def\dopFq#1#2#3#4#5{%
        {}_{#1}F_{#2}\biggl[\genfrac..{0pt}{}{#3}{#4};#5\biggr]%
        \endgroup
}

%------------------------------------
%		JOHAN
%------------------------------------
\safemath{\Rmax}{R^*(n,\epsilon)} %rate without CSIT
\safemath{\codewords}{K}
\safemath{\Rub}{\bar{R}(n,\epsilon)}
\safemath{\Rlb}{\underline{R}(n,\epsilon)}
\safemath{\rk}{\kappa}
\safemath{\rlos}{\bar{\matH}}
\safemath{\rnlos}{\tilde{\randmatH}}

\safemath{\randtemp}{K}

\safemath{\Vnocsit}{V_{\error}^{\mathrm{no}}}
\safemath{\Vcsit}{V_{\error}^{\mathrm{rt}}}

\safemath{\cadist}{F_C} %capacity distribution
\safemath{\cdistno}{F_{0}}
\safemath{\cdistcsit}{F_{1}}


\safemath{\deF}{d_0} %the derivative of F_C(\xi) %\left.\frac{d\cadist(\argpn)}{d\argpn}\right|_{\argpn=C_\error}

\safemath{\bl}{n} %block length
\safemath{\blt}{\tilde{\bl}}
\safemath{\error}{\epsilon} %prob of error
\safemath{\NumCode}{M}
\safemath{\RXant}{r}
%\safemath{\rxant}{r}
%\safemath{\txant}{t}
\safemath{\txantop}{t^{\ast}}
\safemath{\minant}{m}
\safemath{\minantop}{\minant^\ast}
\safemath{\snr}{\rho}
\safemath{\const}{k}
\safemath{\inset}{\setF} %the input power set
\safemath{\spanm}{\mathrm{span}}
\safemath{\ubb}{b_{0}}%upper bound of b_1,...,b_{r} of the matrix I+ H^H U H.

%%%%%%%%%%%MIMO%%%%%%%%%%%%%%%%%%%%
\safemath{\covmat}{\matU}
\safemath{\covmatY}{\matV}
\safemath{\randcmY}{\randmatV}

\safemath{\insetMIMO}{\setF_{\txant,\bl}}
\safemath{\insetcov}{\setU_{\txant}}
%\safemath{\condcov}{\matQ\succeq\mathbf{0},\tr(\matQ)\leq\snr}
\safemath{\condcov}{\matQ\in\insetcov}

\safemath{\BoundFU}{k_{\delta}}

\safemath{\argpn}{\xi} % the argument in the probability p(R)

\safemath{\angletest}{Z} %the angle test used in achievability part

\safemath{\Cnocsit}{C_{\epsilon}^{(0)}}
\safemath{\Ccsit}{C_{\epsilon}^{(1)}}

\safemath{\errorach}{P_\mathrm{e}} %the error in intuition part



\newcommand{\given}{\,\vert\,}				% conditioning
\newcommand{\ggiven}{\,\Vert\,}	
\safemath{\define}{\triangleq}			% definition
%\safemath{\fnorm}{\mathrm{F}}

\safemath{\altbl}{\tilde{\bl}}
\safemath{\constL}{k_{\mathrm{L}}}
\safemath{\constU}{k_{\mathrm{U}}}
\safemath{\funcL}{\tilde{q}}
\safemath{\funcU}{q}
\safemath{\ConstThm}{k_0}
%%%%%%%%%%%%%%%%used in the intuition part %%%%%%%%%%%%%
\safemath{\randrevec}{\randvecy}
\safemath{\revec}{\vecy}
\safemath{\trcwd}{\vecx}
\safemath{\randtrcwd}{\randvecx}
\safemath{\randnoisevec}{\randvecw}
\safemath{\transmitcwd}{\vecx_1} %the transmitted codeword in achievability
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%used in the appendix of proving gamma=C_error + O(1/\bl) %%%%%%%%%%%%%
\safemath{\pickcwdnoch}{\vecx_0} %the chosen codeword x=[P,P,...,P]
\safemath{\pickcwd}{\vecx_0} %the chosen codeword x=[P,P,...,P]

\safemath{\inseqrand}{\randvecx}
\safemath{\inseq}{\vecx}

\safemath{\outseq}{\matY}
\safemath{\outseqrand}{\randmatY}

%used in the appendix of the proof of achievability
\safemath{\altT}{\widetilde{T}}
\safemath{\altU}{\widetilde{U}}
\safemath{\altmean}{\tilde{\mu}}
\safemath{\altvar}{\tilde{\sigma}}
\safemath{\altf}{\funcL}
\safemath{\altg}{\tilde{g}}
\safemath{\altgamma}{\tilde{\gamma}}
\safemath{\altdelta}{\tilde{\delta}}
\safemath{\altk}{\tilde{k}}
\safemath{\altconst}{\altk}
\safemath{\altbmLambda}{\widetilde{\bm{\Lambda}}}
\safemath{\constant}{\tilde{k}}

